Klout Topics for Modeling Interests and Expertise of Users Across Social Networks

This paper presents Klout Topics, a lightweight ontology to describe social media users' topics of interest and expertise. Klout Topics is designed to: be human-readable and consumer-friendly; cover multiple domains of knowledge in depth; and promote data extensibility via knowledge base entities. We discuss why this ontology is well-suited for text labeling and interest modeling applications, and how it compares to available alternatives. We show its coverage against common social media interest sets, and examples of how it is used to model the interests of over 780M social media users on Klout.com. Finally, we open the ontology for external use.

==> ontology paper/texfiles/ontology_abstract.tex <==
This paper presents Klout Topics, a lightweight ontology to describe social media users' topics of interest and expertise. Klout Topics is designed to: be human-readable and consumer-friendly; cover multiple domains of knowledge in depth; and promote data extensibility via knowledge base entities. We discuss why this ontology is well-suited for text labeling and interest modeling applications, and how it compares to available alternatives. We show its coverage against common social media interest sets, and examples of how it is used to model the interests of over 780M social media users on Klout.com. Finally, we open the ontology for external use.

==> ontology paper/texfiles/ontology_alternatives.tex <==
We find that the alternative sources of topic labels fall into the following categories:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{Formal ontologies developed for the Semantic Web such as OpenCyc\footnote{\url{http://opencyc.org/}}, OntoLingua \cite{gruber1992ontolingua}, Schema.org\footnote{\url{http://schema.org/}}, etc.} These are larger and more complex than the social media topic domain requires, and would require extra processing to apply. For example, the OpenCyc node ``Game'' is, among other things, an instance of the ``type of temporally stuff-like thing'', which is a complex category out of the scope of topic modeling tasks. 
\item \textbf{Knowledge bases} such as Wikidata\footnote{\url{https://www.wikidata.org/}}, DBPedia\footnote{\url{http://wiki.dbpedia.org/}}, or YAGO\footnote{\url{http://www.mpi-inf.mpg.de/departments/databases-and-information-systems/research/yago-naga/yago/}}. Knowledge bases are by design very large, and contain many entities that are too general, abstract, or specific to be successfully modeled as interests. 
\item \textbf{Lightweight category sets used for ad targeting such as GoogleAds, Twitter Ads, etc.} These are the closest match for the task of interest modeling, and are quite sufficient for many applications; they are the logical basis for comparison for KT. However, because they are designed to be applied in a self-serve UI by advertisers, they tend to be high-level, limited in size, and contain grab-bag or ``Other''-type categories (e.g., ``Fun and Trivia'') that are not present as topics on social media.
\item \textbf{DMOZ\footnote{\url{https://www.dmoz.org/}} or similar URL catalogs.} Because these are intended to catalog URLs and not social media content, they contain format categories that are out of scope of a topic modeling task (e.g. ``Personal Homepages'').
\item \textbf{Yelp or other business catalogs.} These exclude many non-business topics that are present on social media (e.g., ``Donald Trump'', ``History'').
\item \textbf{Amazon, GoodRelations \cite{good-rel} and other product catalogs.} These exclude many non-product topics that are present on social media (e.g., ``Donald Trump'', ``History'').
\item \textbf{LinkedIn or other catalogs of professional skills.} These exclude many non-professional topics that are popular on social media (``Fan Fiction'').
\end{enumerate}

==> ontology paper/texfiles/ontology_best_practices.tex <==
Through the practice of modeling social media interest and expertise topics on Klout.com, we have identified the following best practices for an interest modeling topic set:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{Contain concepts that can be meaningful interests of a person or topics of a document.} One can reasonably say ``This social media user has in-depth knowledge of geometry'' or ``this article is about geometry'', which implies that ``Geometry'' is a good candidate topic. However, one cannot reasonably say ``This social media user has in-depth knowledge of rectangles'', which tells us that assigning  ``Rectangles'' as a topic will likely be seen as a failure of the modeling application.
\item \textbf{Be limited to topics, rather than text formats, user demographics, or other attributes}. We are supporting the task of determining what a given piece of text is about and then aggregating that topic knowledge to label a social profile; it is out of our scope to determine non-topical attributes of the user or the text.
\item \textbf{Contain sufficient depth and range of concepts to cover the wide variety of topics discussed on social media.} A greater number of distinct, meaningful topics allows for more meaningful targeting or labeling of users. Narrower subcategories such ``Gospel Music'' or ``Affordable Care Act'' can be more useful to an application than higher-level categories like ``Music'' or ``Politics''. 
\item \textbf{Be small enough for ease of maintenance.} While a too-small topic set has limited utility, as discussed above, a very large topic set is challenging to curate. In addition, a very large topic set can be expensive to model over large amounts of social media content. 
\item \textbf{Be up-to-date with topics likely to be discussed on social media.} Certain domains, such as technology, politics and popular culture, evolve rapidly; a topic set from even a year ago is likely to have problematic gaps.
\item \textbf{Be readable by end users.} If the modeled topics are to be exposed in an application, they should be named with clarity and brevity. (e.g., ``Humidifiers'' is preferable to ``Humidifier (Product)'').
\item \textbf{Be structured hierarchically to leverage connections between concepts}. This allows the modeling application to infer knowledge upward in the graph (e.g., to understand that a user who is interested in ``Chicago Cubs'' will also be interested in ``Baseball'').
\item \textbf{Support multiple languages.} A single-language topic set will limit the final application.
\item \textbf{Include knowledge base entity ids, for data extensibility.} Mapping topics to entities in a knowledge base such as Wikipedia or Freebase is useful for a number of NLP tasks, such as entity disambiguation.
\end{enumerate}

==> ontology paper/texfiles/ontology_characteristics.tex <==

\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|}
%\begin{tabular}{|p{4cm}|p{1cm}|p{1cm}|} 
 \hline
 \textbf{Root} & \textbf{Nodes} & \textbf{Edges} \\ [0.5ex] 
 \hline
Arts and Humanities & 565 & 625 \\ \hline
Food and Drink & 268 & 313 \\ \hline
Government and Politics & 484 & 527 \\ \hline
Health and Wellness & 374 & 422 \\ \hline
News and Media & 157 & 164 \\ \hline
Science and Nature & 635 & 623 \\ \hline
Sports and Recreation & 827 & 894 \\ \hline
Location & 912 & 1019 \\ \hline
Fashion & 242 & 259 \\ \hline
Education & 648 & 656 \\ \hline
Hobbies & 92 & 110 \\ \hline
Entertainment & 5779 & 5325 \\ \hline
Business & 809 & 884 \\ \hline
Technology & 1131 & 1196 \\ \hline
Lifestyle & 635 & 681 \\ \hline
Travel and Tourism & 73 & 79 \\ [1ex] 
 \hline
\end{tabular}}
\caption{Root categories of KT, with counts of nodes and edges}
\label{table:1}
\vspace{-0.3in}
\end{table}

We present Klout Topics, a lightweight curated ontology % or associative concept network
designed to model user and text topics across social networks. The latest version can be accessed on GitHub\footnote{\url{https://github.com/klout/opendata/tree/master/klout_topic_ontology}}.

\subsection{Methodology}
KT was initially bootstrapped from a set of 140K Freebase topic nodes, selected by matching popular keywords from social media text. That set was curated down to 20K candidates by removing nodes that were not sufficiently popular on social media (``Australian Desert Raisin'') or not sufficiently intuitive for application use (``Comments''). Relationships within those 20K nodes were then inferred from Freebase and verified by curators. With ongoing curation, KT reached its current size of 8K nodes and 13K edges, with newly relevant topics added and obsolete ones removed.

\subsection{Scope}
As users on social networks interact with a variety of topics and domains, KT aims to include any concept that:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{is specific enough} to meaningfully describe a user's interest or the primary topic of a piece of text (e.g., ``Life'' or ``Growing'' are too broad, but ``Biology'' or ``Child Development'' should be included).
\item \textbf{is general enough} to be shared by a community of interest on social media, with content that can be detected and recommended. A topic that is theoretically possible, but lacks users or content (e.g. ``Scandinavian Death Metal Played on Kazoos'') will not be included.
\item \textbf{is not redundant} with topics already present (``Child Development Milestones'' does not need to be a separate topic from ``Child Development''). 
\item \textbf{is not illegal or offensive} to a general audience.
\end{enumerate}

\subsection{Components and definitions}

\subsubsection{Topic nodes}

Each topic node in KT contains:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{topic\_id}: a unique numerical identifier for the topic. 
\item \textbf{slug}: a human-readable English label, usable in a URL.
\item \textbf{metadata}: includes both the Wikidata entity ID and Freebase machine\_id of the closest corresponding entity. This facilitates NLP tasks such as entity disambiguation and linking  \cite{Bhargava:lithiumnlp}. 
%between similarly-named nodes (such as ``The Vaccines'' [the band] versus ``Vaccines'' [disease-preventing biological preparations]). 
\end{enumerate}

\subsubsection{Topic Edges}
KT is structured as a directed graph %[\ref{fig:graph}], 
with all branches connected to one or more of the 16 root categories in Table \ref{table:1}. 
Each edge indicates a parent-child relationship where a child may be a subclass of the parent (e.g., ``Philosophy'' > ``Ethics''), or a notable entity within the topic context (``Philosophy'' > ``Friedrich Nietzsche''). 
A child may have multiple parents in different branches of the graph, and parents may be at different distances from the root.

Each edge contains:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{edge\_id}: a unique numerical identifier for the edge.
\item \textbf{source\_topic\_id}: the topic\_id of the parent topic.
\item \textbf{destination\_topic\_id}: the topic\_id of the child topic.
\end{enumerate}

%\begin{figure}[t]
%\caption{An example of the directed graph structure of Klout Topics.}
%\centering
%\fbox{\includegraphics[width=0.4\textwidth]{ontology_tree_example}}
%\label{fig:graph}
%\end{figure}

\subsubsection{Topic Display Names}
 
A topic node is associated with the following fields to define how it should be displayed:
\begin{enumerate}[nolistsep,noitemsep]
\item \textbf{topic\_id}: the unique identifier for the topic.
\item \textbf{language}: the language of the given display\_name.
\item \textbf{display\_type}: a flag to indicate whether the topic should be displayed in the given language.
\item \textbf{display\_name}: the most correct and human-readable form of the topic name, in the given language.
\end{enumerate}
In order for KT to be used in consumer-facing applications, its editorial voice strives to be \textbf{transparent} (avoiding neologisms and domain-specific jargon), \textbf{neutral or positive in tone} (avoiding ideological connotations), and \textbf{inclusive} (avoiding derogatory speech and using self-identified terms for groups of people).

\subsection{Internationalization}

A core assumption of KT is that the concept encoded in a node is \textit{not} language- or region-specific, but can be shared across languages. Rather than maintaining separate topic sets for each language, therefore, a single multi-lingual instance can be used. This approach allows for direct comparison of the interests of users in different languages. For flexibility in the application, however, we include a flag to indicate whether a topic should be displayed in a given language.

Currently, the following languages are supported: Arabic (KSA), English (USA), French, German, and Spanish (EU).

% \subsection{Voice and Vocabulary}
% In order for KT to be used in consumer-facing applications, its editorial voice strives to be:
% \begin{itemize}[nolistsep,noitemsep]
% \item \textbf{transparent}: avoiding neologisms and domain-specific jargon when possible; using full names of places and people (``New York City'' instead of ``NYC''). 
% \item \textbf{neutral or positive in tone}: avoiding terms with ideological connotations. In some cases where no neutral term exists (such as ``Gun Control'' and ``Gun Rights''), both versions are included.
% \item \textbf{inclusive}: avoiding derogatory language; when referring groups of people, choosing the most widely used self-identification (``LGBT'' instead of ``Gay'').
% \end{itemize}

==> ontology paper/texfiles/ontology_conclusion.tex <==
In this paper, we have described the importance of a robust topic set for text labeling and topic modeling applications taking input from social media; the topic set should be lightweight, human-readable, span multiple domains of knowledge, and be mapped to a commonly used knowledge base for extensibility to natural language processing tasks. We then discussed the drawbacks of some of the currently available options for this purpose, and proposed Klout Topics (KT) instead. We gave an overview of KT's purpose, characteristics, and coverage; and finally, we gave examples of how it can be used to model a range of topics based on a person's social network activity.


==> ontology paper/texfiles/ontology_in_practice.tex <==
% \begin{itemize}
%   \item Counts of people, URLs, messages, wikis with assigned topics
%   \begin{itemize}
%     \item Rankings of most popular topics for each of the above
%   \end{itemize}
%   \item visualization of counts and rankings on a world map
% \end{itemize}


==> ontology paper/texfiles/ontology_introduction.tex <==
% core argument: the topic/keyword set chosen can impact the success of interest modeling distinct from the accuracy of the model itself

The richness of social media as a source of information about its users' interests and areas of expertise has led to a great deal of research on natural language processing (NLP) algorithms for extracting that data. Taking free-form text and modeling it as structured topics opens up a variety of applications that are not possible with unstructured bags of keywords. However, an often-neglected aspect of the modeling task is choosing \textit{which} set of candidate topics to use. Through the practice of modeling social media interest and expertise topics on Klout.com, we have identified several criteria for such a topic set. These include: 
\begin{itemize}[noitemsep,nolistsep]
\item covering many domains of knowledge in depth and in multiple languages; 
\item being human-readable, so that modeled topics can be exposed by an application;
\item being small enough for human curation to be feasible;
\item containing links from knowledge base entities to topics, to enable NLP tasks.
\end{itemize}
For these reasons, we see that the choice of topic set can have significant implications for the success of a text labeling, topic modeling, or other NLP applications \cite{Bhargava:lithiumnlp}.

To address these challenges, we present Klout Topics (KT), a curated, lightweight ontology of over 8K nodes and over 13K edges, and discuss:
\begin{itemize}[noitemsep,nolistsep]
\item its characteristics and structure,
\item its relative strengths compared to alternatives,
\item its coverage measured against topics used in Twitter Interests\footnote{\url{http://business.twitter.com/en/targeting/interest.html}}and Google Ads\footnote{\url{https: //support.google.com/ads/answer/2842480?hl=en}}, and 
\item case studies applying it to social media profiles.
\end{itemize}

==> ontology paper/texfiles/ontology_lessons_learned.tex <==
\subsection{Overview of Development}

\subsection{Bootstrapping the Ontology}
The first version of the ontology consisted of 140k nodes from the following sources: 
\begin{enumerate}
\item Keywords extracted from processed tweets
\item (Which academic topic sets? need reference) 
\end{enumerate}

A team of employees was tasked with whittling down the set of topics by removing those that were:
\begin{itemize}
\item too specific to be applied to a significant number of profiles or URLs (``Offices of Dentists (Industry)'', ``Australian Desert Raisin (Ingredient)'')
\item too general or ambiguous to be meaningful (``Minister-President'', ``Comments'', ``Short List'')
\item out of date (``Seattle Supersonics (Basketball)'')
\item containing profanity or adult content (``Tits \& Clits Comix (Comic Books)'')
\end{itemize} 
This approach resulted in a set of ~10,000 v1 topics. Each topic node contained a unique numerical identifier, a human-readable string identifier, an English-language display\_name, and a ``type'' field indicating where it lay within the ontology's tree structure (see below).

The same team was then tasked with verifying parent-child relationships inferred from Freebase's data structure. A stand-alone tool was created for this task, which required (time estimate).  

v1 topics were organized into a three-level tree:
\begin{itemize} 
\item Supertopics: 15 top-level domains, e.g. ``Business'' and ``Entertainment''
\item Subtopics: \~1000 more specific categories, such as ``Accounting'' and ``Music''. Each subtopic is limited to a single parent at the supertopic level.
\item Entities: \~9000 named ``entities'' or more specific topics, such as ``TurboTax'' or ``Lady Gaga''. Each entity may have multiple parents, but at the subtopic level only. (todo: clarify definition of entities here versus in Papyrus)
\end{itemize}

A dedicated ontology specialist was brought on to normalize topic names and handle ongoing curation and maintenance. 
This included normalizing names from the formal, parenthesis-heavy academic labels; adding missing topics too new or simply overlooked in Freebase; and deleting duplicate concepts.

v1 of the ontology had several drawbacks. 
First, the three-level limit caused a pile-up at the bottommost (``entity'') level, where topics that should have had a parent-child relationship were forced into a sibling one instead; for example, v1 contained both \textbf{Sports and Recreation > Baseball > Major League Baseball} and \textbf{Sports and Recreation > Baseball > Boston Red Sox}, where the preferred path would be \textbf{Sports and Recreation > Baseball > Major League Baseball > Boston Red Sox}. 
Similarly, the restriction on the allowed level of a parent topic meant that not all possible paths could be represented; the v1 ontology could support either \textbf{Hobbies > Antiques} or \textbf{Lifestyle > Home Decorating > Antiques}, but not both.

An even more pressing problem from a business perspective was that the v1 ontology could only support a single display\_name, and therefore could not be internationalized without supporting multiple parallel versions. 

\subsection{Ontology Development}
Beginning in 2014, we began developing an improved version of the Klout ontology, incorporating the following changes. 
(More about the characteristics of ontology v2 can be found in section 5, below.)

First, v2 removed restrictions on number and level of parent topics, moving from a topic tree to a directed graph. 
We retained the original set of top-level topics, but now allow multiple parents at any level so long as the resulting path is not recursive. 

Next, we added internationalization as an additional dimension of metadata attached to the topic node; now every node includes multiple display\_names in supported languages. 
From both a technical and curation standpoint, we found this approach preferable to maintaining parallel ontologies by language or region. 
While some topics are certainly rooted in a given region or language and will be less frequently found elsewhere (''Toronto Film Festival'', for example), the parent topics will be unchanged, so there is no need to maintain a separate graph. 
Furthermore, adding internationalization to the existing ontology gave us a ``cold start'' for those languages, from which we can work to incrementally improve topic coverage for non-US-English concepts and domains. 
Each display\_name also comes with a flag to indicate whether the given topic should be shown or hidden for the given language, allowing some pruning of less-regionally-relevant topics on the front end.

All internationalization within the ontology is handled at the language level, not the country or other region. 
For business reasons, we also may enforce the hiding of particular topics within particular regions (for example, ``LGBT'' and similar topics within Saudi Arabia). 
However, because those are business decisions that can vary widely by circumstance and application, we chose not to encode those within the ontology itself.

Finally, v2 adds a pointer to the primary Freebase entity for each topic. 
This provides a richer data set for machine learning or text-processing applications.

\subsection{Lessons Learned and Best Practices}
% TODO: revise as advice for others facing similar problems

While much has been written about formal ontology construction, especially for semantic web applications, less has been said about the practical realities of lightweight ontology construction for an enterprise or commercial user-facing application. 
The following are some of the most important lessons learned during the construction, implementation and maintenance of the Klout topic ontology.

\textbf{Expectation of Curation and Incremental Change}. 
An ontology is a living knowledge artifact; it must be clear throughout the organization that building one requires an ongoing investment in the form of time, tools, and documentation. 
Even when choosing to adopt an externally created ontology, it's crucial to consider when and how to propogate updates, whether they come from the external ontology's original creators, or from inside one's own organization. 

\textbf{Clear Chain of Ownership and Documentation}. 
Because an ontology is a living artifact, it should be clear what teams or persons have the authority to make changes. Those owners should document the principles used to make changes, addressing the ontology's scope, structure, and voice. 
A transparent historical record of changes to the ontology is also recommended.

\textbf{Limiting Assumptions}. 
Encoding too many assumptions into your ontology can be dangerous, especially when it spans multiple domains. 
As we saw above, v1 of the Klout ontology was unsatisfactory in part because it assumed both that the top-level categories were mutually exclusive and that there was no need for a path longer than three nodes. 
Fewer rules to enforce can, paradoxically, lead to a cleaner ontology, as well as saving development and curation time.

\textbf{Inclusivity and Tone}. 
Especially if your ontology will be used to visibly classify persons, it is a matter of business importance to be as inclusive as possible. 
Your ontology will reflect your organization's values in the eyes of many users. 
Strive for both caution and consistency when dealing with ideologically controversial concepts, adult concepts, and so forth.

\textbf{Storage Formats and Tools for Curation}. 
There are a range of approaches to storing and describing ontologies, from OWL and Protege, to XTM topic maps, to simple tables in SQL and similar databases. (TODO: Add references) Because ours is a lightweight ontology with a single relationship type, and to make it easier to integrate our ontology with the rest of the data processing pipeline, we chose the straightforward table method, with some temporary front-end tools spun up when needed. This tradeoff has often required the rules of the ontology to be enforced by curators rather than within the tool, emphasizing the importance of clear documentation and quality assurance (see below).

\subsubsection{Metrics and Quality Assurance}.
Like any feature, an ontology in active use should be monitored for quality issues. 
However, it can be difficult to quantify an ontology's issues apart from those of its application. 
When maintaining the Klout ontology, we consider the following:

\textbf{Coverage, a.k.a. Missing Topics}. 
Misapplied topics application can indicate a gap in the ontology, where a less appropriate or too general topic is being used for lack of a better alternative. 
Topics that are missing because they are new concepts can often be identified through current news and tools like Google Trends.

\textbf{Scope, a.k.a. Unneeded Topics}. 
Topics not being applied in the application are often topics that are unneeded. 
Some of these will be topics that were once relevant but are now obsolete and can be safely ``aged out'' of the ontology. 
This is especially true of constantly evolving areas like consumer electronics, movies and television.

\textbf{Missing and Incorrect Edges}. 
Detecting missing or incorrect edges is one of the most difficult areas of ontology improvement. 
Because the Klout ontology does encode references to Freebase, we can compare our edges to Freebase and to some extent to Wikipedia.

\textbf{Application Metrics and User Feedback}. 
Application-level metrics are undeniably useful, although some investigation is required to determine when the cause lies in the ontology and when it lies in some other part of the application. 
There should be a clear path for user feedback about topic assignments.

\textbf{Validation Against Other Ontologies}. 
Validating against other available ontologies is time-consuming, since it requires aligning the ontologies to be compared, but can be revealing. 
See Section 6.

==> ontology paper/texfiles/ontology_other_ontologies.tex <==
% \begin{itemize}
%   \item address: OpenCyc, Google ads/news, Twitter, Yelp, OpenCyc, Freebase, Wiki categories, some academic publishing ontology (old)
%   \item address: LI skills, TW lists, URL meta tags -- todo: find something equivalent for FB
%   \item qualitative aspects not present in other candidate ontologies (e.g. language agnosticism, entity mapping, granularity and ability to support deep paths)
%   \item metrics and visualizations for: 
%   \begin{enumerate}
%     \item scope/coverage (Venn/overlap)
%     \begin{enumerate}
%       \item high-level: overlap of subject domains
%       \item overlap on particular topics
%     \end{enumerate}
%     \item specificity/depth (e.g. number of children for a given concept)
%     \begin{enumerate}
%       \item depth of tree (allows inferred information, unlike flag tag structured th)
%       \item numbers of children
%     \end{enumerate}    
%     \item structure
%     \begin{enumerate}
%       \item types of connections available
%       \item overlap of hierarchical connections
%     \end{enumerate} 
%     \item application level TBD?
%     \item ease of adoption/integration? (simple structure, relatively few tables, etc.)
%     \item extensibility
%     \item evolvability
%     \item interoperability (can modelling done with an alternative ontology be compared to modelling done with our ontology)
%     \item clarity/coherence/readability
%   \end{enumerate}
% \end{itemize}

% Table generated by running:
% com.lithium.text.graph.GraphIOUtilTest located at
% //code/text/text-core/src/test/java/com/lithium/text/graph/GraphIOUtilTest.java

\begin{table*}
\center
\begin{tabular}{ |c|l|l|l|l|}
\hline
 & KLOUT & GOOGLE\_ADS & EBAY\_US & OPEN\_CYC \\ \hline
NODE\_COUNT & 7623 & 8005 & 18022 & 119941 \\ \hline
EDGE\_COUNT & 12958 & 2023 & 17988 & 184990 \\ \hline
HAS\_CYCLES & 0 & 0 & 0 & 1 \\ \hline
CYCLE\_COUNT & 0 & 0 & 0 & 187 \\ \hline
IS\_COUNT & 0 & 0 & 0 & 0 \\ \hline
CONNECTED\_SET\_COUNT & 12 & 5982 & 34 & 5687 \\ \hline
VERTEX\_DEGRE\_AVERAGE & 3.4 & 0.51 & 2 & 3.08 \\ \hline
VERTEX\_IN\_DEGREE\_AVERAGE & 1.7 & 0.25 & 1 & 1.54 \\ \hline
VERTEX\_OUT\_DEGREE\_AVERAGE & 1.7 & 0.25 & 1 & 1.54 \\ \hline
MAX\_PATH\_SIZE & 5 & 4 & 5 & 18 \\ \hline
GRAPH\_DISTANCE & 1.4 & 1.19 & 2.28 & 5.61 \\ \hline
CLOSENESS\_CENTRALITY & 0.26 & 0.31 & 0.2 & 0.06 \\ \hline
\end{tabular}
\caption{Various Graph Related Metrics on Ontologyies}\label{table:onthology_metrics}
\end{table*}




==> ontology paper/texfiles/ontology_problem_statement.tex <==
How can the choice of a candidate topic set impact the success of an interest modeling application? Consider the topics that could be assigned to the Twitter profile of machine learning expert Andrew Ng\footnote{\url{http://twitter.com/AndrewYNg}}. For an interest modeling application to assign meaningful labels to this profile, it would need a topic set containing concepts like ``AI'', ``Coursera'', and ``Stanford''. But is there value in representing ``AI'' and ``Artifical Intelligence'' as distinct topics? Should the topic set contain entities like ``Baidu AI Group'', and would we expect them to be successfully modeled? Should the topic set contain abstract concepts like ``Thought'' or ``Power'', and would those convey any meaning when assigned? If the topic set included negatively-viewed concepts such as ``Terrorist Propaganda'' or ``Spam'', and those topics were assigned based on a post like Figure \ref{fig:andrewng}, would we risk implying that the user is either a terrorist or a spammer? These risks increase when modeling interests over large numbers of social media profiles, and make it advisable to use a carefully curated topic set.

\begin{figure}[t]
\centering
\includegraphics[scale=0.15]{andrewng}
\caption{Tweet by Andrew Ng, 18 June 2017}
\label{fig:andrewng}
\vspace{-0.1in}
\end{figure}

==> ontology paper/texfiles/ontology_related.tex <==
\cite{nemanja-lasta} is always a related file.


==> ontology paper/texfiles/ontology_results.tex <==

% \begin{figure*}
% \centering
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{topic_distribution_LI_PROFILE_1_DAY_GENERATED}
%   \caption{LinkedIn PROFILE}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{topic_distribution_LI_SKILLZ_1_DAY_GENERATED}
%   \caption{LinkedIn SKILLZ}
%   \label{fig:sub2}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{topic_distribution_LI_INDUSTRY_1_DAY_GENERATED}
%   \caption{LinkedIn INDUSTRY}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Distribution of users-labels mapping to top-layer topics}
% \label{fig:test}
% \end{figure*}

\begin{table} [t]
\begin{minipage}[b]{1\linewidth} 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|}%{|p{1.75cm}|p{1.75cm}|p{1.75cm}|p{1.75cm}|}
 \hline
 \textbf{Frequent Interest} & \textbf{Rare Interest} & \textbf{Frequent Expertise} & \textbf{Rare Expertise} \\
 \hline
 Social Media & Unisys & Twitter & Unisys \\
  \hline
 Twitter & Andalusia & Music & Andalusia \\
  \hline
 Music & AstraZeneca & Actors & AstraZeneca \\
   \hline
 Actors & Quebec City & Celebrities & Big Band \\
   \hline
 Software & Inbound Marketing & Media & Apulia \\
   \hline
 Television & Category Theory & Sports & Biotelemetry \\
   \hline
 Internet & Dreamworks & YouTube & Infusium \\
   \hline
 Sports & Marketing Automation & Soccer & Inbound Marketing \\
   \hline
 Media & Biotelemetry & Entertainment & Category Theory \\
   \hline
 Celebrities & Objective-J & Singing & Biolage \\
   \hline
 YouTube & Stridex & Internet & Objective-J \\
   \hline
 Entertainment & Cloudera Impala & Television & Stridex \\
   \hline
 Film & Assisted Living & Humor & Dreamworks \\
   \hline
 Humor & Bavaria & Politics & Marketing Automation \\
   \hline
 Politics & Tajikistan & Portugal & Sketch Comedy \\
   \hline
\end{tabular}}
\caption{Frequently and infrequently assigned Klout Topics.}
\label{table:3}
\end{minipage}
\begin{minipage}[b]{1\linewidth} 
\centering
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|}
 \hline
 & \textbf{KT} & \textbf{Twitter} & \textbf{Google} \\
 \hline
 Top-level & 16 & 25 & 11 \\
 \hline
 Nodes & 8028 & 350 & 2042 \\ 
 \hline
 Depth & 6 & 2 & 9 \\
 \hline
\end{tabular}}
\caption{KT size and depth vs. Twitter and Google interests.}
\label{table:2}
\end{minipage}
\begin{minipage}[b]{1\linewidth} 
\centering
\scalebox{0.77}{
\begin{tabular}{|p{3.5cm}|p{3.5cm}|}
 \hline
 \textbf{Interest} & \textbf{Expertise} \\
 \hline
 Twitter & Twitter \\
   \hline
 YouTube & YouTube \\
   \hline
 Feminism & Singing \\
   \hline
 Singing & Islam \\
   \hline
 Donald Trump & Feminism \\
   \hline
 Islam & Mecca \\
   \hline
 Leadership & Donald Trump \\
   \hline
 MTV & Riyadh \\
   \hline
 Inspiration & MTV \\
   \hline
 Facebook & Justin Bieber \\
   \hline
 One Direction & Inspiration \\
   \hline
 Instagram & Instagram \\
   \hline
 Nature & K-Pop \\
   \hline
 SnapChat & CNN \\
   \hline
 LGBT & LGBT \\
   \hline
\end{tabular}}
\caption{Frequent Klout Topics not in Twitter or Google sets.}
\label{table:4}
\vspace{-0.3in}
\end{minipage}
\end{table}

Here we discuss how the coverage of Klout Topics compares to other topic sets used for modeling user interests. Table \ref{table:2} compares the topical coverage of KT versus Twitter Interests\cite{twitter-ads} and Google ad categories\cite{google-ads}.
While the number of top-level categories is comparable across all three, KT contains the most overall nodes, as well as a significantly deeper structure than Twitter Interests and a comparable one to Google Ads.

In practice, Klout Topics also allows us to model both widely-shared and relatively narrow interests. Table \ref{table:3} shows a sample of Klout Topics assigned to 50M or more profiles out of over 780M scored on Klout.com (``Frequent Interest/Expertise''), as well as a sample of Klout Topics assigned to 10K or fewer (``Rare Interest/Expertise''), as of June 2017. 

Table \ref{table:4} shows popular Klout Topics (assigned to 10M or more profiles as of late June 2017) that are not present in either the Twitter or Google sets. Other examples of topics unique to KT include some brands (``Converse'', ``Pizza Hut''), news-driven concepts (``Affordable Care Act'', ``Criminal Justice Reform''), and narrow subconcepts  (``West Papua'' in addition to ``Indonesia'', ``Aquariums'' in addition to ``Zoos'', ``DevOps'' in addition to ``Programming''). Conversely, Table \ref{table:5} shows a sample of Twitter and Google topics not present in KT. Analysis finds 24 Twitter and 154 Google topics not represented in some form in KT. Many of these missing topics are product subtypes (``Women's Beachwear'') or categories of URLs (``Skins Themes and Wallpapers'').

\begin{table} [t]
\begin{minipage}[b]{1\linewidth} 
\centering
\scalebox{0.78}{
\begin{tabular}{|c|c|}
%\begin{tabular}{|p{3.5cm}|p{3.5cm}|}
 \hline
 \textbf{Twitter} & \textbf{Google} \\
  \hline
   Dresses and skirts & ATMs and Branch Locations \\
  \hline
     Empty nesters & Bottled Water \\
  \hline
     Kids' apparel & Clip Art and Animated GIFs \\
  % \hline
     % Men's accessories & Ink and Toner \\
  \hline
     Men's beachwear & Men's Interests \\
  \hline
     Venues & Offbeat \\
  \hline
     Women's accessories & Puzzles and Brainteasers \\
  % \hline
     % Women's bags & Sleepwear \\
  \hline
     Women's beachwear & Song Lyrics and Tabs \\
  \hline
     Women's jeans & Special Occasions \\
  % \hline
  %    Women's outerwear & Temporary and Seasonal Jobs \\
  \hline
     Women's pants & Vacation Offers \\
  % \hline
  %    Women's shoes & Valentine's Day \\
  \hline
     Women's tops & World Localities \\
  \hline
\end{tabular}}
\caption{Sample Twitter and Google interests not in KT.}
\label{table:5}
\vspace{-0.3in}
\end{minipage}
% \begin{minipage}[b]{1\linewidth} 
% \centering
% \scalebox{0.8}{
% \begin{tabular}{|p{7cm}|}
%  \hline
%  \textbf{OpenCyc nodes} \\
%  \hline
%  Sulfite \\
%    \hline
%  DroneAttacksInPakistan \\
%    \hline
%  Pentaerythritol \\
%    \hline
%  ArabianRedFox \\
%    \hline
%  Lettuce\_sandwich \\
%    \hline
%  GlassSquid \\
%    \hline
%  RefractiveEyeSurgery \\
%    \hline
%  Water\_soluble\_signaling\_molecule \\
%    \hline
%  NonPhysicianMedicalCareProfessional \\
%    \hline
% \end{tabular}}
% \caption{Sample OpenCyc nodes not present in KT.}
% \label{table:6}
% \vspace{-0.2in}
% \end{minipage}
\end{table}

% Table \ref{table:6} shows a random sample of nodes from OpenCyc that are not present in KT. Many OpenCyc nodes are too specific to be usefully modeled as interests (``Lettuce\_sandwich'', ``Water\_soluble\_signaling\_molecule'').

% Although we cannot compare the size and structure of the Klout Topic Ontology to LinkedIn skills because LinkedIn does not expose its full ontology, Figure 1 shows a mapping between skills found in LinkedIn profiles from Klout consumers and the Klout Topic Ontology, where Klout topics are aggregated to the root level. The bias toward the Business and Technology portions of the graph are what one would expect, given LinkedIn's focus on professional skills.

==> ontology paper/texfiles/ontology_sample_case_study.tex <==

\begin{figure}[t]
\centering
\begin{subfigure}{0.45\textwidth}
\includegraphics[scale=0.35]{andrewng2}
\caption{Klout Topics on the Klout.com profile of Andrew Ng}
\label{fig:andrewng2}
\end{subfigure} 
\centering
\begin{subfigure}{0.45\textwidth}
\includegraphics[scale=0.35]{kamalaharris}
\caption{Klout Topics on the Klout.com profile of Kamala Harris}
\label{fig:kamalaharris}
\end{subfigure} 
\centering
\begin{subfigure}{0.45\textwidth}
\includegraphics[scale=0.35]{sarahellinger}
\caption{Klout Topics on the Klout.com profile of Sarah Ellinger}
\label{fig:sarahellinger}
\vspace{-0.1in}
\end{subfigure} 
\caption{Klout Topics on sample user profiles from Klout.com}
\label{fig:klouitprofiles}
\vspace{-0.2in}
\end{figure}


% \begin{table} [t]
% \begin{minipage}[b]{1\linewidth} 
% \centering
% \scalebox{0.75}{
% \begin{tabular}{|c|c|}
%  \hline
%  \textbf{Interest} & \textbf{Expertise} \\
%   \hline
%     Barack Obama & United States of America \\
%   \hline
%     Politics & Barack Obama \\
%   \hline
%     United States of America & Politics \\
%   \hline
%     CNN & Government \\
%   \hline
%     Health & Internet \\
%   \hline
%     Chicago & Religion \\
%   \hline
%     Republican Party & Telecommunications \\
%   \hline
%     Washington DC & Activism \\
%   \hline
%     New York City & History \\
%   \hline
%     Communications & Washington DC \\
%   \hline
%     Innovation & Chicago \\
%   \hline
%     Donald Trump & Healthcare Reform \\
%   \hline
%     Media & Michelle Obama \\
%   \hline
% \end{tabular}}
% \caption{Top-scoring topics for \@BarackObama on Twitter.}
% \label{table:7}
% \end{minipage}
% \begin{minipage}[b]{1\linewidth} 
% \centering
% \scalebox{0.75}{
% \begin{tabular}{|c|c|}
%  \hline
%  \textbf{Interest} & \textbf{Expertise} \\
%   \hline
%     Actors & Actors \\
%   \hline
%     Donald Trump & Celebrities \\
%   \hline
%     Film & New York City \\
%   \hline
%     New York City & Activism \\
%   \hline
%     Politics & Children \\
%   \hline
%     Hydraulic Fracturing & Film Production \\
%   \hline
%     Academy Awards & Marvel Comics \\
%   \hline
%     Los Angeles & Thor \\
%   \hline
%     The Environment & The Avengers \\
%   \hline
%     Entertainment & Movies \\
%   \hline
%     Democratic Party & Hydraulic Fracturing \\
%   \hline
%     Russia & Democracy Now \\
%   \hline
%     Republican Party & Agents of S.H.I.E.L.D \\
%   \hline\end{tabular}}
% \caption{Top-scoring topics for \@MarkRuffalo on Twitter.}
% \label{table:8}
% \end{minipage}
% \begin{minipage}[b]{1\linewidth} 
% \centering
% \scalebox{0.75}{
% \begin{tabular}{|c|c|}
%  \hline
%  \textbf{Interest} & \textbf{Expertise} \\
%   \hline
%      Politics & Internet \\
%   \hline
%      Copyright Law & Technology \\
%   \hline
%       Internet & Law \\
%   \hline
%       U.S. Supreme Court & Privacy \\
%   \hline
%       Donald Trump & Activism \\
%   \hline
%       Republican Party & Software \\
%   \hline
%       United States Congress & Barack Obama \\
%   \hline
%       Creative Commons & Copyright Law \\
%   \hline
%       Harvard University & Democracy \\
%   \hline
%       Barack Obama & Net Neutrality \\
%   \hline
%       Democratic Party & U.S. Supreme Court \\
%   \hline
%       Activism & Creative Commons \\
%   \hline
%       Campaign Finance & Radio Frequency \\
%   \hline
%   \end{tabular}}
% \caption{Top-scoring topics for \@lessig on Twitter.}
% \label{table:9}
% \vspace{-0.2in}
% \end{minipage}
% \end{table}


Here, we show examples of how KT is used to model expertise topics of over 780M social media users on Klout.com, using the Klout topic assignment system (\cite{nemanja-lasta}, \cite{spasojevic2016mining}). These topic scores are also available via the Twitter PowerTrack API\footnote{\url{http://support.gnip.com/apis/powertrack/}}.

Figure [\ref{fig:andrewng2}] shows the expertise topics displayed on the Klout.com profile of Andrew Ng, which range from the broad (``Computer Science'') to the relatively narrow (``Apache Spark''). Figure [\ref{fig:kamalaharris}] shows the Klout.com profile of Senator Kamala Harris, and includes many topics specific to her state of California as well as some relating to government and politics. Figure [\ref{fig:sarahellinger}] shows the Klout.com profile of one of the authors of this paper, and includes a mix of modeled expertise topics (``Eventbrite'', ``Klout'') as well as non-modeled topics from KT that the user has selected (``Parenting'').

==> texfiles/ontology_in_practice.tex <==
% \begin{itemize}
%   \item Counts of people, URLs, messages, wikis with assigned topics
%   \begin{itemize}
%     \item Rankings of most popular topics for each of the above
%   \end{itemize}
%   \item visualization of counts and rankings on a world map
% \end{itemize}


==> texfiles/ontology_lessons_learned.tex <==
\subsection{Overview of Development}

\subsection{Bootstrapping the Ontology}
The first version of the ontology consisted of 140k nodes from the following sources: 
\begin{enumerate}
\item Keywords extracted from processed tweets
\item (Which academic topic sets? need reference) 
\end{enumerate}

A team of employees was tasked with whittling down the set of topics by removing those that were:
\begin{itemize}
\item too specific to be applied to a significant number of profiles or URLs (``Offices of Dentists (Industry)'', ``Australian Desert Raisin (Ingredient)'')
\item too general or ambiguous to be meaningful (``Minister-President'', ``Comments'', ``Short List'')
\item out of date (``Seattle Supersonics (Basketball)'')
\item containing profanity or adult content (``Tits \& Clits Comix (Comic Books)'')
\end{itemize} 
This approach resulted in a set of ~10,000 v1 topics. Each topic node contained a unique numerical identifier, a human-readable string identifier, an English-language display\_name, and a ``type'' field indicating where it lay within the ontology's tree structure (see below).

The same team was then tasked with verifying parent-child relationships inferred from Freebase's data structure. A stand-alone tool was created for this task, which required (time estimate).  

v1 topics were organized into a three-level tree:
\begin{itemize} 
\item Supertopics: 15 top-level domains, e.g. ``Business'' and ``Entertainment''
\item Subtopics: \~1000 more specific categories, such as ``Accounting'' and ``Music''. Each subtopic is limited to a single parent at the supertopic level.
\item Entities: \~9000 named ``entities'' or more specific topics, such as ``TurboTax'' or ``Lady Gaga''. Each entity may have multiple parents, but at the subtopic level only. (todo: clarify definition of entities here versus in Papyrus)
\end{itemize}

A dedicated ontology specialist was brought on to normalize topic names and handle ongoing curation and maintenance. 
This included normalizing names from the formal, parenthesis-heavy academic labels; adding missing topics too new or simply overlooked in Freebase; and deleting duplicate concepts.

v1 of the ontology had several drawbacks. 
First, the three-level limit caused a pile-up at the bottommost (``entity'') level, where topics that should have had a parent-child relationship were forced into a sibling one instead; for example, v1 contained both \textbf{Sports and Recreation > Baseball > Major League Baseball} and \textbf{Sports and Recreation > Baseball > Boston Red Sox}, where the preferred path would be \textbf{Sports and Recreation > Baseball > Major League Baseball > Boston Red Sox}. 
Similarly, the restriction on the allowed level of a parent topic meant that not all possible paths could be represented; the v1 ontology could support either \textbf{Hobbies > Antiques} or \textbf{Lifestyle > Home Decorating > Antiques}, but not both.

An even more pressing problem from a business perspective was that the v1 ontology could only support a single display\_name, and therefore could not be internationalized without supporting multiple parallel versions. 

\subsection{Ontology Development}
Beginning in 2014, we began developing an improved version of the Klout ontology, incorporating the following changes. 
(More about the characteristics of ontology v2 can be found in section 5, below.)

First, v2 removed restrictions on number and level of parent topics, moving from a topic tree to a directed graph. 
We retained the original set of top-level topics, but now allow multiple parents at any level so long as the resulting path is not recursive. 

Next, we added internationalization as an additional dimension of metadata attached to the topic node; now every node includes multiple display\_names in supported languages. 
From both a technical and curation standpoint, we found this approach preferable to maintaining parallel ontologies by language or region. 
While some topics are certainly rooted in a given region or language and will be less frequently found elsewhere (''Toronto Film Festival'', for example), the parent topics will be unchanged, so there is no need to maintain a separate graph. 
Furthermore, adding internationalization to the existing ontology gave us a ``cold start'' for those languages, from which we can work to incrementally improve topic coverage for non-US-English concepts and domains. 
Each display\_name also comes with a flag to indicate whether the given topic should be shown or hidden for the given language, allowing some pruning of less-regionally-relevant topics on the front end.

All internationalization within the ontology is handled at the language level, not the country or other region. 
For business reasons, we also may enforce the hiding of particular topics within particular regions (for example, ``LGBT'' and similar topics within Saudi Arabia). 
However, because those are business decisions that can vary widely by circumstance and application, we chose not to encode those within the ontology itself.

Finally, v2 adds a pointer to the primary Freebase entity for each topic. 
This provides a richer data set for machine learning or text-processing applications.

\subsection{Lessons Learned and Best Practices}
% TODO: revise as advice for others facing similar problems

While much has been written about formal ontology construction, especially for semantic web applications, less has been said about the practical realities of lightweight ontology construction for an enterprise or commercial user-facing application. 
The following are some of the most important lessons learned during the construction, implementation and maintenance of the Klout topic ontology.

\textbf{Expectation of Curation and Incremental Change}. 
An ontology is a living knowledge artifact; it must be clear throughout the organization that building one requires an ongoing investment in the form of time, tools, and documentation. 
Even when choosing to adopt an externally created ontology, it's crucial to consider when and how to propogate updates, whether they come from the external ontology's original creators, or from inside one's own organization. 

\textbf{Clear Chain of Ownership and Documentation}. 
Because an ontology is a living artifact, it should be clear what teams or persons have the authority to make changes. Those owners should document the principles used to make changes, addressing the ontology's scope, structure, and voice. 
A transparent historical record of changes to the ontology is also recommended.

\textbf{Limiting Assumptions}. 
Encoding too many assumptions into your ontology can be dangerous, especially when it spans multiple domains. 
As we saw above, v1 of the Klout ontology was unsatisfactory in part because it assumed both that the top-level categories were mutually exclusive and that there was no need for a path longer than three nodes. 
Fewer rules to enforce can, paradoxically, lead to a cleaner ontology, as well as saving development and curation time.

\textbf{Inclusivity and Tone}. 
Especially if your ontology will be used to visibly classify persons, it is a matter of business importance to be as inclusive as possible. 
Your ontology will reflect your organization's values in the eyes of many users. 
Strive for both caution and consistency when dealing with ideologically controversial concepts, adult concepts, and so forth.

\textbf{Storage Formats and Tools for Curation}. 
There are a range of approaches to storing and describing ontologies, from OWL and Protege, to XTM topic maps, to simple tables in SQL and similar databases. (TODO: Add references) Because ours is a lightweight ontology with a single relationship type, and to make it easier to integrate our ontology with the rest of the data processing pipeline, we chose the straightforward table method, with some temporary front-end tools spun up when needed. This tradeoff has often required the rules of the ontology to be enforced by curators rather than within the tool, emphasizing the importance of clear documentation and quality assurance (see below).

\subsubsection{Metrics and Quality Assurance}.
Like any feature, an ontology in active use should be monitored for quality issues. 
However, it can be difficult to quantify an ontology's issues apart from those of its application. 
When maintaining the Klout ontology, we consider the following:

\textbf{Coverage, a.k.a. Missing Topics}. 
Misapplied topics application can indicate a gap in the ontology, where a less appropriate or too general topic is being used for lack of a better alternative. 
Topics that are missing because they are new concepts can often be identified through current news and tools like Google Trends.

\textbf{Scope, a.k.a. Unneeded Topics}. 
Topics not being applied in the application are often topics that are unneeded. 
Some of these will be topics that were once relevant but are now obsolete and can be safely ``aged out'' of the ontology. 
This is especially true of constantly evolving areas like consumer electronics, movies and television.

\textbf{Missing and Incorrect Edges}. 
Detecting missing or incorrect edges is one of the most difficult areas of ontology improvement. 
Because the Klout ontology does encode references to Freebase, we can compare our edges to Freebase and to some extent to Wikipedia.

\textbf{Application Metrics and User Feedback}. 
Application-level metrics are undeniably useful, although some investigation is required to determine when the cause lies in the ontology and when it lies in some other part of the application. 
There should be a clear path for user feedback about topic assignments.

\textbf{Validation Against Other Ontologies}. 
Validating against other available ontologies is time-consuming, since it requires aligning the ontologies to be compared, but can be revealing. 
See Section 6.

==> texfiles/ontology_other_ontologies.tex <==
% \begin{itemize}
%   \item address: OpenCyc, Google ads/news, Twitter, Yelp, OpenCyc, Freebase, Wiki categories, some academic publishing ontology (old)
%   \item address: LI skills, TW lists, URL meta tags -- todo: find something equivalent for FB
%   \item qualitative aspects not present in other candidate ontologies (e.g. language agnosticism, entity mapping, granularity and ability to support deep paths)
%   \item metrics and visualizations for: 
%   \begin{enumerate}
%     \item scope/coverage (Venn/overlap)
%     \begin{enumerate}
%       \item high-level: overlap of subject domains
%       \item overlap on particular topics
%     \end{enumerate}
%     \item specificity/depth (e.g. number of children for a given concept)
%     \begin{enumerate}
%       \item depth of tree (allows inferred information, unlike flag tag structured th)
%       \item numbers of children
%     \end{enumerate}    
%     \item structure
%     \begin{enumerate}
%       \item types of connections available
%       \item overlap of hierarchical connections
%     \end{enumerate} 
%     \item application level TBD?
%     \item ease of adoption/integration? (simple structure, relatively few tables, etc.)
%     \item extensibility
%     \item evolvability
%     \item interoperability (can modelling done with an alternative ontology be compared to modelling done with our ontology)
%     \item clarity/coherence/readability
%   \end{enumerate}
% \end{itemize}

% Table generated by running:
% com.lithium.text.graph.GraphIOUtilTest located at
% //code/text/text-core/src/test/java/com/lithium/text/graph/GraphIOUtilTest.java

\begin{table*}
\center
\begin{tabular}{ |c|l|l|l|l|}
\hline
 & KLOUT & GOOGLE\_ADS & EBAY\_US & OPEN\_CYC \\ \hline
NODE\_COUNT & 7623 & 8005 & 18022 & 119941 \\ \hline
EDGE\_COUNT & 12958 & 2023 & 17988 & 184990 \\ \hline
HAS\_CYCLES & 0 & 0 & 0 & 1 \\ \hline
CYCLE\_COUNT & 0 & 0 & 0 & 187 \\ \hline
IS\_COUNT & 0 & 0 & 0 & 0 \\ \hline
CONNECTED\_SET\_COUNT & 12 & 5982 & 34 & 5687 \\ \hline
VERTEX\_DEGRE\_AVERAGE & 3.4 & 0.51 & 2 & 3.08 \\ \hline
VERTEX\_IN\_DEGREE\_AVERAGE & 1.7 & 0.25 & 1 & 1.54 \\ \hline
VERTEX\_OUT\_DEGREE\_AVERAGE & 1.7 & 0.25 & 1 & 1.54 \\ \hline
MAX\_PATH\_SIZE & 5 & 4 & 5 & 18 \\ \hline
GRAPH\_DISTANCE & 1.4 & 1.19 & 2.28 & 5.61 \\ \hline
CLOSENESS\_CENTRALITY & 0.26 & 0.31 & 0.2 & 0.06 \\ \hline
\end{tabular}
\caption{Various Graph Related Metrics on Ontologyies}\label{table:onthology_metrics}
\end{table*}




==> texfiles/ontology_related.tex <==
\cite{nemanja-lasta} is always a related file.

